Local Similarity Search on Geolocated Time Series Using Hybrid Indexing

Geolocated time series, i.e., time series associated with certain locations, abound in many modern applications. In this paper, we consider hybrid queries for retrieving geolocated time series based on filters that combine spatial distance and time series similarity. For the latter, unlike existing work, we allow filtering based on local similarity, which is computed based on subsequences rather than the entire length of each series, thus allowing the discovery of more fine-grained trends and patterns. To efficiently support such queries, we first leverage the state-of-the-art BTSR-tree index, which utilizes bounds over both the locations and the shapes of time series to prune the search space. Moreover, we propose optimizations that check at specific timestamps to identify candidate time series that may exceed the required local similarity threshold. To further increase pruning power, we introduce the SBTSR-tree index, an extension to BTSR-tree, which additionally segments the time series temporally, allowing the construction of tighter bounds. Our experimental results on several real-world datasets demonstrate that SBTSR-tree can provide answers much faster for all examined query types. This paper has been published in the 27th International Conference on Advances in Geographic Information Systems (ACM SIGSPATIAL 2019).

==> test.tex <==




% \begin{minipage}{.25\textwidth}

% \begin{figure*}[htbp]
% \centering
% \subfloat{\fbox{\includegraphics[width=0.35\textwidth]{Figures/legend.png}}}
% \\
% \vspace{-5pt}
% \subfloat[Crime ($Q_{rr}$)]{\includegraphics[trim=0.5cm 0.5cm 0.5cm 0.5cm, clip, width=0.225\textwidth]{Figures/Plots/Crime/varying_delta.eps}\label{subfig:var_delta_crime}}
% \subfloat[Crime ($Q_{kr}$)]{\includegraphics[trim=0.5cm 0.5cm 0.5cm 0.5cm, clip, width=0.225\textwidth]{Figures/Plots/Crime/varying_k_query2.eps}\label{subfig:var_k_crime}}
% \subfloat[Crime ($Q_{rk}$)]{\includegraphics[trim=0.5cm 0.5cm 0.5cm 0.5cm, clip, width=0.225\textwidth]{Figures/Plots/Crime/varying_k_query3.eps}\label{subfig:var_ks_crime}}
% \subfloat[$Q_{rr}$]{\includegraphics[trim=0.5cm 0.5cm 0.5cm 0.5cm, clip, width=0.225\textwidth]{Figures/Plots/Scalability/varyingDatasetSize_1.eps}\label{subfig:scalability1}} \\
% \vspace{-5pt}
% \subfloat[Flickr ($Q_{rr}$)]{\includegraphics[trim=0.5cm 0.5cm 0.5cm 0.5cm, clip, width=0.225\textwidth]{Figures/Plots/Flickr/varying_delta.eps}\label{subfig:var_delta_flickr}}
% \subfloat[Flickr ($Q_{kr}$)]{\includegraphics[trim=0.5cm 0.5cm 0.5cm 0.5cm, clip, width=0.225\textwidth]{Figures/Plots/Flickr/varying_k_query2.eps}\label{subfig:var_k_flickr}}
% \subfloat[Flickr ($Q_{rk}$)]{\includegraphics[trim=0.5cm 0.5cm 0.5cm 0.5cm, clip, width=0.225\textwidth]{Figures/Plots/Flickr/varying_k_query3.eps}\label{subfig:var_ks_flickr}}
% \subfloat[$Q_{kr}$]{\includegraphics[trim=0.5cm 0.5cm 0.5cm 0.5cm, clip, width=0.225\textwidth]{Figures/Plots/Scalability/varyingDatasetSize_2.eps}\label{subfig:scalability2}} \\
% \vspace{-5pt}
% \subfloat[Taxi ($Q_{rr}$)]{\includegraphics[trim=0.5cm 0.5cm 0.5cm 0.5cm, clip, width=0.225\textwidth]{Figures/Plots/Taxi/varying_delta.eps}\label{subfig:var_delta_taxi}}
% \subfloat[Taxi ($Q_{kr}$)]{\includegraphics[trim=0.5cm 0.5cm 0.5cm 0.5cm, clip, width=0.225\textwidth]{Figures/Plots/Taxi/varying_k_query2.eps}\label{subfig:var_k_taxi}}
% \subfloat[Taxi ($Q_{rk}$)]{\includegraphics[trim=0.5cm 0.5cm 0.5cm 0.5cm, clip, width=0.225\textwidth]{Figures/Plots/Taxi/varying_k_query3.eps}\label{subfig:var_ks_taxi}}
% \subfloat[$Q_{rk}$]{\includegraphics[trim=0.5cm 0.5cm 0.5cm 0.5cm, clip, width=0.225\textwidth]{Figures/Plots/Scalability/varyingDatasetSize_3.eps}\label{subfig:scalability3}}
% \vspace{-5pt}
% \caption{Per column: $Q_{rr}(T_q, \rho, \epsilon, \delta)$ for varying $\delta$ -- $Q_{kr}(T_q, k, \epsilon, \delta)$ -- $Q_{rk}(T_q, k, \rho)$ for varying $k$ -- scalability. }
% \label{fig:exp}
% \end{figure*}

% \end{minipage}


% \begin{figure*}[htbp]
% \centering
% \subfloat{\fbox{\includegraphics[width=0.35\textwidth]{Figures/legend.png}}}\end{figure*}


% \begin{figure*}
% \centering
% \begin{minipage}[h]{0.24\linewidth}
% \subfigure[Crime ($Q_{rr}$)]{\includegraphics[trim=0.5cm 0.5cm 0.5cm 0.5cm, clip, width=0.9\textwidth]{Figures/Plots/Crime/varying_delta.eps}\label{subfig:var_delta_crime}} \\
% \subfigure[Flickr ($Q_{rr}$)]{\includegraphics[trim=0.5cm 0.5cm 0.5cm 0.5cm, clip, width=0.9\textwidth]{Figures/Plots/Flickr/varying_delta.eps}\label{subfig:var_delta_flickr}} \\
% \subfigure[Taxi ($Q_{rr}$)]{\includegraphics[trim=0.5cm 0.5cm 0.5cm 0.5cm, clip, width=0.9\textwidth]{Figures/Plots/Taxi/varying_delta.eps}\label{subfig:var_delta_taxi}}
% % \caption{$Q_{rr}(T_q, \rho, \epsilon, \delta)$ for varying $\delta$}\label{exp:triggerings}
% \end{minipage}

% \begin{minipage}[h]{0.24\linewidth}
% \subfigure[Crime ($Q_{kr}$)]{\includegraphics[trim=0.5cm 0.5cm 0.5cm 0.5cm, clip, width=0.9\textwidth]{Figures/Plots/Crime/varying_k_query2.eps}\label{subfig:var_k_crime}} \\
% \subfigure[Flickr ($Q_{kr}$)]{\includegraphics[trim=0.5cm 0.5cm 0.5cm 0.5cm, clip, width=0.9\textwidth]{Figures/Plots/Flickr/varying_k_query2.eps}\label{subfig:var_k_flickr}} \\
% \subfigure[Taxi ($Q_{kr}$)]{\includegraphics[trim=0.5cm 0.5cm 0.5cm 0.5cm, clip, width=0.9\textwidth]{Figures/Plots/Taxi/varying_k_query2.eps}\label{subfig:var_k_taxi}}
% % \caption{$Q_{kr}(T_q, k, \epsilon, \delta)$}\label{exp:stage_cost}
% \end{minipage}

% \begin{minipage}[h]{0.24\linewidth}
% \subfigure[Crime ($Q_{rk}$)]{\includegraphics[trim=0.5cm 0.5cm 0.5cm 0.5cm, clip, width=0.225\textwidth]{Figures/Plots/Crime/varying_k_query3.eps}\label{subfig:var_ks_crime}} \\
% \subfigure[Flickr ($Q_{rk}$)]{\includegraphics[trim=0.5cm 0.5cm 0.5cm 0.5cm, clip, width=0.225\textwidth]{Figures/Plots/Flickr/varying_k_query3.eps}\label{subfig:var_ks_flickr}} \\
% \subfigure[Taxi ($Q_{rk}$)]{\includegraphics[trim=0.5cm 0.5cm 0.5cm 0.5cm, clip, width=0.225\textwidth]{Figures/Plots/Taxi/varying_k_query3.eps}\label{subfig:var_ks_taxi}}
% % \caption{$Q_{rk}(T_q, k, \rho)$ for varying $k$}\label{exp:histogram}
% \end{minipage}

% \begin{minipage}[h]{0.24\linewidth}
% \subfigure[$Q_{rr}$]{\includegraphics[trim=0.5cm 0.5cm 0.5cm 0.5cm, clip, width=0.225\textwidth]{Figures/Plots/Scalability/varyingDatasetSize_1.eps}\label{subfig:scalability1}} \\
% \subfigure[$Q_{kr}$]{\includegraphics[trim=0.5cm 0.5cm 0.5cm 0.5cm, clip, width=0.225\textwidth]{Figures/Plots/Scalability/varyingDatasetSize_2.eps}\label{subfig:scalability2}} \\
% \subfigure[$Q_{rk}$]{\includegraphics[trim=0.5cm 0.5cm 0.5cm 0.5cm, clip, width=0.225\textwidth]{Figures/Plots/Scalability/varyingDatasetSize_3.eps}\label{subfig:scalability3}}
% % \caption{Scalability}\label{exp:histogram}
% \end{minipage}

% \end{figure*}



\begin{figure*}
\centering

\begin{minipage}[h]{0.32\linewidth}
{\subfigure[$Q_{rk}$]{\includegraphics[trim=0.5cm 0.5cm 0.5cm 0.5cm, clip, width=0.9\textwidth]{Figures/Plots/Crime/varying_delta.eps}\label{subfig:scalability3}}}\label{exp:triggerings} 
{\subfigure[$Q_{rk}$]{\includegraphics[trim=0.5cm 0.5cm 0.5cm 0.5cm, clip, width=0.9\textwidth]{Figures/Plots/Flickr/varying_delta.eps}\label{subfig:scalability3}}}\label{exp:triggerings} 
{\subfigure[$Q_{rk}$]{\includegraphics[trim=0.5cm 0.5cm 0.5cm 0.5cm, clip, width=0.9\textwidth]{Figures/Plots/Taxi/varying_delta.eps}\label{subfig:scalability3}}}\label{exp:triggerings}
\caption{Processing cost per stage}\label{exp:stage_cost}
\end{minipage}


\begin{minipage}[h]{0.32\linewidth}
{\subfigure[$Q_{rk}$]{\includegraphics[trim=0.5cm 0.5cm 0.5cm 0.5cm, clip, width=0.9\textwidth]{Figures/Plots/Scalability/varyingDatasetSize_3.eps}\label{subfig:scalability3}}}\label{exp:triggerings} 
{\subfigure[$Q_{rk}$]{\includegraphics[trim=0.5cm 0.5cm 0.5cm 0.5cm, clip, width=0.9\textwidth]{Figures/Plots/Scalability/varyingDatasetSize_3.eps}\label{subfig:scalability3}}}\label{exp:triggerings} 
{\subfigure[$Q_{rk}$]{\includegraphics[trim=0.5cm 0.5cm 0.5cm 0.5cm, clip, width=0.9\textwidth]{Figures/Plots/Taxi/varying_delta.eps}\label{subfig:scalability3}}}\label{exp:triggerings}
\caption{Processing cost per stage}\label{exp:stage_cost}
\end{minipage}

\begin{minipage}[h]{0.32\linewidth}
{\subfigure[$Q_{rk}$]{\includegraphics[trim=0.5cm 0.5cm 0.5cm 0.5cm, clip, width=0.9\textwidth]{Figures/Plots/Scalability/varyingDatasetSize_3.eps}\label{subfig:scalability3}}}\label{exp:triggerings} 
{\subfigure[$Q_{rk}$]{\includegraphics[trim=0.5cm 0.5cm 0.5cm 0.5cm, clip, width=0.9\textwidth]{Figures/Plots/Scalability/varyingDatasetSize_3.eps}\label{subfig:scalability3}}}\label{exp:triggerings} 
{\subfigure[$Q_{rk}$]{\includegraphics[trim=0.5cm 0.5cm 0.5cm 0.5cm, clip, width=0.9\textwidth]{Figures/Plots/Taxi/varying_delta.eps}\label{subfig:scalability3}}}\label{exp:triggerings}
\caption{Active trajectories per cycle}\label{exp:histogram}
\end{minipage}

\end{figure*}

